Optimal Per-Antenna ADC Bit Allocation in Correlated and Cell-Free Massive MIMO

In Massive MIMO base stations (BSs), the hardware design needs to balance high spectral efficiency (SE) with low complexity. The level of hardware impairments (HWIs) indicates how strong the signal distortion introduced by hardware imperfections is. In particular, the analog-to-digital converters (ADCs) have an important impact on signal distortion and power consumption. This article addresses the fundamental problem of selecting the optimal hardware quality in the Massive MIMO space. In particular, we examine the optimal HWI and ADC bit allocation per BS antenna to maximize the SE. The results show that in co-located arrays with low channel gain variations across antennas, equal ADC bit allocation is optimal. In contrast, cell-free Massive MIMO systems benefit the most from optimizing the ADC bit allocation achieving improvements in the order of 2 [bit-per-channel-use] per user equipment when using regularized zero-forcing (RZF). In addition, when including the impact of power consumption in cell-free Massive MIMO with RZF, allocating low values of mixed ADC bit resolutions across the BS antennas can increase the energy efficiency up to 30% compared to equal ADC bit allocation.

==> Figures/CDF_EqQbit_MR.tex <==
% !TeX root = ../HWI_OP_draft.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8


\begin{tikzpicture}
	%\usetikzlibrary{arrows}
	\begin{axis}[
	width=0.47\textwidth,
	height=0.32\textwidth,
	y label style = {at={(-0.03,0.5)},anchor=north},
	xlabel={SE per UE [bpcu]},
	ylabel={CDF},
%	extra y ticks={2},
%	extra y tick labels={2},% \footnotesize
%	extra x ticks={25},
%	extra x tick labels={25},		
	xmin = 0,
	xmax =5,
	ymin = 0,
	ymax = 1,
%	xtick distance = 100,
%	ytick distance = 10,
	line width = 1pt,
	grid=both,
	legend columns = 1,
%	transpose legend,
	%	 legend pos= north west,%(0.44,0.99)
%	legend style={at={(axis cs: 600,1.35)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	legend style={at={(axis cs: 5,0.55)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	]	

% ============== LEGEND ===================

	\addlegendentry{Co-corr-I}	
	\addlegendimage{black, mark=square, solid,mark options={solid, line width = 0.8pt},mark size=2pt}	
	\addlegendentry{Co-corr-D1}	
	\addlegendimage{red, mark=triangle,    densely dashed,mark options={solid, line width = 0.8pt},mark size=2pt}
	\addlegendentry{Co-corr-DK}
	\addlegendimage{green, mark=x,    dashdotdotted,mark options={solid, line width = 0.9pt},mark size=2.3pt}
	\addlegendentry{Cell-free}	
	\addlegendimage{blue, mark=o,    densely dotted,mark options={solid, line width = 0.8pt},mark size=2pt}
% ============== PLOTS ===================
% All results are for M = 100

% MR  Eq - ADC - CoI 
	\addplot [black, mark=square, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={1}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% MR  Eq - unCorr - CoI 
\addplot [black, mark=none, solid]%,xindexrange={3}{5} 		
table[x index={33}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
			   %4
% MR  Eq - ADC - CoD1								
	\addplot [red, mark=triangle, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={5}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			
					
% MR  Eq - unCorr - CoD1
	\addplot [red, mark=none,    densely dashed]%,xindexrange={3}{5} 		
	table[x index={34}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			
					%10			
	
% MR  Eq - ADC - CoDK								
	\addplot [green, mark=x, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.9pt},mark size=2.5pt]%,xindexrange={3}{5} 		
	table[x index={9}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
% MR  Eq - unCorr - CoDK
	\addplot [green, mark=none,    dashdotdotted]%,xindexrange={3}{5} 		
	table[x index={35}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
					%16



% MR  Eq - ADC - Cfree 
\addplot [blue, mark=o,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
table[x index={13}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% MR  Eq - unCorr - Cfree 
\addplot [blue, mark=none, densely dotted]%,xindexrange={3}{5} 		
table[x index={36}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
				%22
%			green!60!black





%% MR  Eq 
%\addplot [gray, mark=+,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
%table[x index={1}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
%\addplot [gray, mark=none, line width = 0.7pt, solid]%,xindexrange={3}{5} 		
%table[x index={33}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
%
%% RZF  Eq 
%\addplot [gray, mark=+,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
%table[x index={2}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
%\addplot [gray, mark=none, line width = 0.7pt, solid]%,xindexrange={3}{5} 		
%table[x index={4}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};

	\end{axis}
	\end{tikzpicture}%

% (0)Percentile					(1)MR-Hw-Eq-PwFx-ADC-CoI	(2)RZF-Hw-Eq-PwFx-ADC-CoI		(3)MR-Hw-Eq-PwFx-unC-CoI	(4)RZF-Hw-Eq-PwFx-unC-CoI		(5)MR-Hw-Eq-PwFx-ADC-CoD1	(6)RZF-Hw-Eq-PwFx-ADC-CoD1		(7)MR-Hw-Eq-PwFx-unC-CoD1	(8)RZF-Hw-Eq-PwFx-unC-CoD1		(9)MR-Hw-Eq-PwFx-ADC-CoDK	(10)RZF-Hw-Eq-PwFx-ADC-CoDK		(11)MR-Hw-Eq-PwFx-unC-CoDK	(12)RZF-Hw-Eq-PwFx-unC-CoDK		(13)MR-Hw-Eq-PwFx-ADC-Cfree	(14)RZF-Hw-Eq-PwFx-ADC-Cfree	(15)MR-Hw-Eq-PwFx-unC-Cfree	(16)RZF-Hw-Eq-PwFx-unC-Cfree	(17)MR-Hw-mPi-PwFx-ADC-CoI	(18)RZF-Hw-mPi-PwFx-ADC-CoI		(19)MR-Hw-mPi-PwFx-unC-CoI	(20)RZF-Hw-mPi-PwFx-unC-CoI		(21)MR-Hw-mPi-PwFx-ADC-CoD1	(22)RZF-Hw-mPi-PwFx-ADC-CoD1	(23)MR-Hw-mPi-PwFx-unC-CoD1	(24)RZF-Hw-mPi-PwFx-unC-CoD1	(25)MR-Hw-mPi-PwFx-ADC-CoDK	(26)RZF-Hw-mPi-PwFx-ADC-CoDK	(27)MR-Hw-mPi-PwFx-unC-CoDK	(28)RZF-Hw-mPi-PwFx-unC-CoDK	(29)MR-Hw-mPi-PwFx-ADC-Cfree	(30)RZF-Hw-mPi-PwFx-ADC-Cfree	(31)MR-Hw-mPi-PwFx-unC-Cfree	(32)RZF-Hw-mPi-PwFx-unC-Cfree	(33)Cl_form-Hw-Eq-PwFx--CoI	(34)Cl_form-Hw-Eq-PwFx--CoD1	(35)Cl_form-Hw-Eq-PwFx--CoDK	(36)Cl_form-Hw-Eq-PwFx--Cfree	(37)Cl_form-Hw-mPi-PwFx--CoI	(38)Cl_form-Hw-mPi-PwFx--CoD1	(39)Cl_form-Hw-mPi-PwFx--CoDK	(40)Cl_form-Hw-mPi-PwFx--Cfree	

%=========================================================

%   (0)Percentile					(1)M=100MR-Eq-bit-ADC-CoI			(2)M=100RZF-Eq-bit-ADC-CoI			(3)M=100SMMSE-Eq-bit-ADC-CoI	(4)M=100MR-Eq-bit-unC-CoI			(5)M=100RZF-Eq-bit-unC-CoI			(6)M=100SMMSE-Eq-bit-unC-CoI		(7)M=100MR-Eq-bit-ADC-CoD1	(8)M=100RZF-Eq-bit-ADC-CoD1			(9)M=100SMMSE-Eq-bit-ADC-CoD1		(10)M=100MR-Eq-bit-unC-CoD1			(11)M=100RZF-Eq-bit-unC-CoD1	(12)M=100SMMSE-Eq-bit-unC-CoD1		(13)M=100MR-Eq-bit-ADC-CoDK			(14)M=100RZF-Eq-bit-ADC-CoDK		(15)M=100SMMSE-Eq-bit-ADC-CoDK	(16)M=100MR-Eq-bit-unC-CoDK			(17)M=100RZF-Eq-bit-unC-CoDK		(18)M=100SMMSE-Eq-bit-unC-CoDK		(19)M=100MR-Eq-bit-ADC-Cfree	(20)M=100RZF-Eq-bit-ADC-Cfree		(21)M=100SMMSE-Eq-bit-ADC-Cfree		(22)M=100MR-Eq-bit-unC-Cfree		(23)M=100RZF-Eq-bit-unC-Cfree	(24)M=100SMMSE-Eq-bit-unC-Cfree		(25)M=100MR-min_pilot-ADC-CoI		(26)M=100RZF-min_pilot-ADC-CoI		(27)M=100SMMSE-min_pilot-ADC-CoI	(28)M=100MR-min_pilot-unC-CoI		(29)M=100RZF-min_pilot-unC-CoI		(30)M=100SMMSE-min_pilot-unC-CoI	(31)M=100MR-min_pilot-ADC-CoD1	(32)M=100RZF-min_pilot-ADC-CoD1		(33)M=100SMMSE-min_pilot-ADC-CoD1	(34)M=100MR-min_pilot-unC-CoD1		(35)M=100RZF-min_pilot-unC-CoD1	(36)M=100SMMSE-min_pilot-unC-CoD1	(37)M=100MR-min_pilot-ADC-CoDK		(38)M=100RZF-min_pilot-ADC-CoDK		(39)M=100SMMSE-min_pilot-ADC-CoDK	(40)M=100MR-min_pilot-unC-CoDK		(41)M=100RZF-min_pilot-unC-CoDK		(42)M=100SMMSE-min_pilot-unC-CoDK	(43)M=100MR-min_pilot-ADC-Cfree	(44)M=100RZF-min_pilot-ADC-Cfree	(45)M=100SMMSE-min_pilot-ADC-Cfree	(46)M=100MR-min_pilot-unC-Cfree		(47)M=100RZF-min_pilot-unC-Cfree	(48)M=100SMMSE-min_pilot-unC-Cfree	(49)M=100Cl_form-Eq-bit--CoI		(50)M=100Cl_form-Eq-bit--CoD1		(51)M=100Cl_form-Eq-bit--CoDK	(52)M=100Cl_form-Eq-bit--Cfree		(53)M=100Cl_form-min_pilot--CoI		(54)M=100Cl_form-min_pilot--CoD1	(55)M=100Cl_form-min_pilot--CoDK	(56)M=100Cl_form-min_pilot--Cfree	

==> Figures/CDF_EqQbit_RZF.tex <==
% !TeX root = ../HWI_OP_draft.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8


\begin{tikzpicture}
	%\usetikzlibrary{arrows}
	\begin{axis}[
	width=0.47\textwidth,
	height=0.32\textwidth,
	y label style = {at={(-0.03,0.5)},anchor=north},
	xlabel={SE per UE [bpcu]},
	ylabel={CDF},
%	extra y ticks={2},
%	extra y tick labels={2},% \footnotesize
%	extra x ticks={25},
%	extra x tick labels={25},		
	xmin = 0,
	xmax =6,
	ymin = 0,
	ymax = 1,
%	xtick distance = 100,
%	ytick distance = 10,
	line width = 1pt,
	grid=both,
	legend columns = 1,
%	transpose legend,
	%	 legend pos= north west,%(0.44,0.99)
%	legend style={at={(axis cs: 600,1.35)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	legend style={at={(axis cs: 2.5,0.95)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	]	

% ============== LEGEND ===================

	\addlegendentry{Co-corr-I}	
	\addlegendimage{black, mark=square, solid,mark options={solid, line width = 0.8pt},mark size=2pt}	
	\addlegendentry{Co-corr-D1}	
	\addlegendimage{red, mark=triangle,    densely dashed,mark options={solid, line width = 0.8pt},mark size=2pt}
	\addlegendentry{Co-corr-DK}
	\addlegendimage{green, mark=x,    dashdotdotted,mark options={solid, line width = 0.9pt},mark size=2.3pt}
	\addlegendentry{Cell-free}	
	\addlegendimage{blue, mark=o,    densely dotted,mark options={solid, line width = 0.8pt},mark size=2pt}
% ============== PLOTS ===================
% All results are for M = 100

% RZF  Eq - ADC - CoI 
	\addplot [black, mark=square, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={2}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% RZF  Eq - unCorr - CoI 
\addplot [black, mark=none, solid]%,xindexrange={3}{5} 		
table[x index={4}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
				
% RZF  Eq - ADC - CoD1								
	\addplot [red, mark=triangle, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={6}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			

% RZF  Eq - unCorr - CoD1
	\addplot [red, mark=none,    densely dashed]%,xindexrange={3}{5} 		
	table[x index={8}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			


% RZF  Eq - ADC - CoDK								
	\addplot [green, mark=x, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.9pt},mark size=2.5pt]%,xindexrange={3}{5} 		
	table[x index={10}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
% RZF  Eq - unCorr - CoDK
	\addplot [green, mark=none,    dashdotdotted]%,xindexrange={3}{5} 		
	table[x index={12}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	




% RZF  Eq - ADC - Cfree 
\addplot [blue, mark=o,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
table[x index={14}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% RZF  Eq - unCorr - Cfree 
\addplot [blue, mark=none, densely dotted]%,xindexrange={3}{5} 		
table[x index={16}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
%			green!60!black

	\end{axis}
	\end{tikzpicture}%

%   (0)Percentile				(1)MR-Hw-Eq-PwFx-ADC-CoI	(2)RZF-Hw-Eq-PwFx-ADC-CoI		(3)MR-Hw-Eq-PwFx-unC-CoI	(4)RZF-Hw-Eq-PwFx-unC-CoI		(5)MR-Hw-Eq-PwFx-ADC-CoD1	(6)RZF-Hw-Eq-PwFx-ADC-CoD1		(7)MR-Hw-Eq-PwFx-unC-CoD1	(8)RZF-Hw-Eq-PwFx-unC-CoD1		(9)MR-Hw-Eq-PwFx-ADC-CoDK	(10)RZF-Hw-Eq-PwFx-ADC-CoDK		(11)MR-Hw-Eq-PwFx-unC-CoDK	(12)RZF-Hw-Eq-PwFx-unC-CoDK		(13)MR-Hw-Eq-PwFx-ADC-Cfree	(14)RZF-Hw-Eq-PwFx-ADC-Cfree	(15)MR-Hw-Eq-PwFx-unC-Cfree	(16)RZF-Hw-Eq-PwFx-unC-Cfree	(17)MR-Hw-mPi-PwFx-ADC-CoI	(18)RZF-Hw-mPi-PwFx-ADC-CoI		(19)MR-Hw-mPi-PwFx-unC-CoI	(20)RZF-Hw-mPi-PwFx-unC-CoI		(21)MR-Hw-mPi-PwFx-ADC-CoD1	(22)RZF-Hw-mPi-PwFx-ADC-CoD1	(23)MR-Hw-mPi-PwFx-unC-CoD1	(24)RZF-Hw-mPi-PwFx-unC-CoD1	(25)MR-Hw-mPi-PwFx-ADC-CoDK	(26)RZF-Hw-mPi-PwFx-ADC-CoDK	(27)MR-Hw-mPi-PwFx-unC-CoDK	(28)RZF-Hw-mPi-PwFx-unC-CoDK	(29)MR-Hw-mPi-PwFx-ADC-Cfree	(30)RZF-Hw-mPi-PwFx-ADC-Cfree	(31)MR-Hw-mPi-PwFx-unC-Cfree	(32)RZF-Hw-mPi-PwFx-unC-Cfree	(33)Cl_form-Hw-Eq-PwFx--CoI	(34)Cl_form-Hw-Eq-PwFx--CoD1	(35)Cl_form-Hw-Eq-PwFx--CoDK	(36)Cl_form-Hw-Eq-PwFx--Cfree	(37)Cl_form-Hw-mPi-PwFx--CoI	(38)Cl_form-Hw-mPi-PwFx--CoD1	(39)Cl_form-Hw-mPi-PwFx--CoDK	(40)Cl_form-Hw-mPi-PwFx--Cfree	

%==============================================
%   (0)Percentile					(1)M=100MR-Eq-bit-ADC-CoI			(2)M=100RZF-Eq-bit-ADC-CoI			(3)M=100SMMSE-Eq-bit-ADC-CoI	(4)M=100MR-Eq-bit-unC-CoI			(5)M=100RZF-Eq-bit-unC-CoI			(6)M=100SMMSE-Eq-bit-unC-CoI		(7)M=100MR-Eq-bit-ADC-CoD1	(8)M=100RZF-Eq-bit-ADC-CoD1			(9)M=100SMMSE-Eq-bit-ADC-CoD1		(10)M=100MR-Eq-bit-unC-CoD1			(11)M=100RZF-Eq-bit-unC-CoD1	(12)M=100SMMSE-Eq-bit-unC-CoD1		(13)M=100MR-Eq-bit-ADC-CoDK			(14)M=100RZF-Eq-bit-ADC-CoDK		(15)M=100SMMSE-Eq-bit-ADC-CoDK	(16)M=100MR-Eq-bit-unC-CoDK			(17)M=100RZF-Eq-bit-unC-CoDK		(18)M=100SMMSE-Eq-bit-unC-CoDK		(19)M=100MR-Eq-bit-ADC-Cfree	(20)M=100RZF-Eq-bit-ADC-Cfree		(21)M=100SMMSE-Eq-bit-ADC-Cfree		(22)M=100MR-Eq-bit-unC-Cfree		(23)M=100RZF-Eq-bit-unC-Cfree	(24)M=100SMMSE-Eq-bit-unC-Cfree		(25)M=100MR-min_pilot-ADC-CoI		(26)M=100RZF-min_pilot-ADC-CoI		(27)M=100SMMSE-min_pilot-ADC-CoI	(28)M=100MR-min_pilot-unC-CoI		(29)M=100RZF-min_pilot-unC-CoI		(30)M=100SMMSE-min_pilot-unC-CoI	(31)M=100MR-min_pilot-ADC-CoD1	(32)M=100RZF-min_pilot-ADC-CoD1		(33)M=100SMMSE-min_pilot-ADC-CoD1	(34)M=100MR-min_pilot-unC-CoD1		(35)M=100RZF-min_pilot-unC-CoD1	(36)M=100SMMSE-min_pilot-unC-CoD1	(37)M=100MR-min_pilot-ADC-CoDK		(38)M=100RZF-min_pilot-ADC-CoDK		(39)M=100SMMSE-min_pilot-ADC-CoDK	(40)M=100MR-min_pilot-unC-CoDK		(41)M=100RZF-min_pilot-unC-CoDK		(42)M=100SMMSE-min_pilot-unC-CoDK	(43)M=100MR-min_pilot-ADC-Cfree	(44)M=100RZF-min_pilot-ADC-Cfree	(45)M=100SMMSE-min_pilot-ADC-Cfree	(46)M=100MR-min_pilot-unC-Cfree		(47)M=100RZF-min_pilot-unC-Cfree	(48)M=100SMMSE-min_pilot-unC-Cfree	(49)M=100Cl_form-Eq-bit--CoI		(50)M=100Cl_form-Eq-bit--CoD1		(51)M=100Cl_form-Eq-bit--CoDK	(52)M=100Cl_form-Eq-bit--Cfree		(53)M=100Cl_form-min_pilot--CoI		(54)M=100Cl_form-min_pilot--CoD1	(55)M=100Cl_form-min_pilot--CoDK	(56)M=100Cl_form-min_pilot--Cfree	

==> Figures/CDF_minPilotQbit_MR.tex <==
% !TeX root = ../HWI_OP_draft.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8


\begin{tikzpicture}
	%\usetikzlibrary{arrows}
	\begin{axis}[
	width=0.47\textwidth,
	height=0.32\textwidth,
	y label style = {at={(-0.03,0.5)},anchor=north},
	xlabel={SE per UE [bpcu]},
	ylabel={CDF},
%	extra y ticks={2},
%	extra y tick labels={2},% \footnotesize
%	extra x ticks={25},
%	extra x tick labels={25},		
	xmin = 0,
	xmax =5,
	ymin = 0,
	ymax = 1,
%	xtick distance = 100,
%	ytick distance = 10,
	line width = 1pt,
	grid=both,
	legend columns = 1,
%	transpose legend,
	%	 legend pos= north west,%(0.44,0.99)
%	legend style={at={(axis cs: 600,1.35)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	legend style={at={(axis cs: 5,0.55)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	]	

% ============== LEGEND ===================

	\addlegendentry{Co-corr-I}	
	\addlegendimage{black, mark=square, solid,mark options={solid, line width = 0.8pt},mark size=2pt}	
	\addlegendentry{Co-corr-D1}	
	\addlegendimage{red, mark=triangle,    densely dashed,mark options={solid, line width = 0.8pt},mark size=2pt}
	\addlegendentry{Co-corr-DK}
	\addlegendimage{green, mark=x,    dashdotdotted,mark options={solid, line width = 0.9pt},mark size=2.3pt}
	\addlegendentry{Cell-free}	
	\addlegendimage{blue, mark=o,    densely dotted,mark options={solid, line width = 0.8pt},mark size=2pt}
% ============== PLOTS ===================
% All results are for M = 100

% MR  Eq - ADC - CoI 
	\addplot [black, mark=square, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={17}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% MR  Eq - unCorr - CoI 
\addplot [black, mark=none, solid]%,xindexrange={3}{5} 		
table[x index={37}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
				%28
% MR  Eq - ADC - CoD1								
	\addplot [red, mark=triangle, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={21}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			

% MR  Eq - unCorr - CoD1
	\addplot [red, mark=none,    densely dashed]%,xindexrange={3}{5} 		
	table[x index={38}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			
					%34

% MR  Eq - ADC - CoDK								
	\addplot [green, mark=x, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.9pt},mark size=2.5pt]%,xindexrange={3}{5} 		
	table[x index={25}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
% MR  Eq - unCorr - CoDK
	\addplot [green, mark=none,    dashdotdotted]%,xindexrange={3}{5} 		
	table[x index={39}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
					%40



% MR  Eq - ADC - Cfree 
\addplot [blue, mark=o,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
table[x index={29}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% MR  Eq - unCorr - Cfree 
\addplot [blue, mark=none, densely dotted]%,xindexrange={3}{5} 		
table[x index={40}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
				%46
%			green!60!black

	\end{axis}
	\end{tikzpicture}%
%   (0)Percentile				(1)MR-Hw-Eq-PwFx-ADC-CoI	(2)RZF-Hw-Eq-PwFx-ADC-CoI		(3)MR-Hw-Eq-PwFx-unC-CoI	(4)RZF-Hw-Eq-PwFx-unC-CoI		(5)MR-Hw-Eq-PwFx-ADC-CoD1	(6)RZF-Hw-Eq-PwFx-ADC-CoD1		(7)MR-Hw-Eq-PwFx-unC-CoD1	(8)RZF-Hw-Eq-PwFx-unC-CoD1		(9)MR-Hw-Eq-PwFx-ADC-CoDK	(10)RZF-Hw-Eq-PwFx-ADC-CoDK		(11)MR-Hw-Eq-PwFx-unC-CoDK	(12)RZF-Hw-Eq-PwFx-unC-CoDK		(13)MR-Hw-Eq-PwFx-ADC-Cfree	(14)RZF-Hw-Eq-PwFx-ADC-Cfree	(15)MR-Hw-Eq-PwFx-unC-Cfree	(16)RZF-Hw-Eq-PwFx-unC-Cfree	(17)MR-Hw-mPi-PwFx-ADC-CoI	(18)RZF-Hw-mPi-PwFx-ADC-CoI		(19)MR-Hw-mPi-PwFx-unC-CoI	(20)RZF-Hw-mPi-PwFx-unC-CoI		(21)MR-Hw-mPi-PwFx-ADC-CoD1	(22)RZF-Hw-mPi-PwFx-ADC-CoD1	(23)MR-Hw-mPi-PwFx-unC-CoD1	(24)RZF-Hw-mPi-PwFx-unC-CoD1	(25)MR-Hw-mPi-PwFx-ADC-CoDK	(26)RZF-Hw-mPi-PwFx-ADC-CoDK	(27)MR-Hw-mPi-PwFx-unC-CoDK	(28)RZF-Hw-mPi-PwFx-unC-CoDK	(29)MR-Hw-mPi-PwFx-ADC-Cfree	(30)RZF-Hw-mPi-PwFx-ADC-Cfree	(31)MR-Hw-mPi-PwFx-unC-Cfree	(32)RZF-Hw-mPi-PwFx-unC-Cfree	(33)Cl_form-Hw-Eq-PwFx--CoI	(34)Cl_form-Hw-Eq-PwFx--CoD1	(35)Cl_form-Hw-Eq-PwFx--CoDK	(36)Cl_form-Hw-Eq-PwFx--Cfree	(37)Cl_form-Hw-mPi-PwFx--CoI	(38)Cl_form-Hw-mPi-PwFx--CoD1	(39)Cl_form-Hw-mPi-PwFx--CoDK	(40)Cl_form-Hw-mPi-PwFx--Cfree		
	
%==========================================================
%   (0)Percentile					(1)M=100MR-Eq-bit-ADC-CoI			(2)M=100RZF-Eq-bit-ADC-CoI			(3)M=100SMMSE-Eq-bit-ADC-CoI	(4)M=100MR-Eq-bit-unC-CoI			(5)M=100RZF-Eq-bit-unC-CoI			(6)M=100SMMSE-Eq-bit-unC-CoI		(7)M=100MR-Eq-bit-ADC-CoD1	(8)M=100RZF-Eq-bit-ADC-CoD1			(9)M=100SMMSE-Eq-bit-ADC-CoD1		(10)M=100MR-Eq-bit-unC-CoD1			(11)M=100RZF-Eq-bit-unC-CoD1	(12)M=100SMMSE-Eq-bit-unC-CoD1		(13)M=100MR-Eq-bit-ADC-CoDK			(14)M=100RZF-Eq-bit-ADC-CoDK		(15)M=100SMMSE-Eq-bit-ADC-CoDK	(16)M=100MR-Eq-bit-unC-CoDK			(17)M=100RZF-Eq-bit-unC-CoDK		(18)M=100SMMSE-Eq-bit-unC-CoDK		(19)M=100MR-Eq-bit-ADC-Cfree	(20)M=100RZF-Eq-bit-ADC-Cfree		(21)M=100SMMSE-Eq-bit-ADC-Cfree		(22)M=100MR-Eq-bit-unC-Cfree		(23)M=100RZF-Eq-bit-unC-Cfree	(24)M=100SMMSE-Eq-bit-unC-Cfree		(25)M=100MR-min_pilot-ADC-CoI		(26)M=100RZF-min_pilot-ADC-CoI		(27)M=100SMMSE-min_pilot-ADC-CoI	(28)M=100MR-min_pilot-unC-CoI		(29)M=100RZF-min_pilot-unC-CoI		(30)M=100SMMSE-min_pilot-unC-CoI	(31)M=100MR-min_pilot-ADC-CoD1	(32)M=100RZF-min_pilot-ADC-CoD1		(33)M=100SMMSE-min_pilot-ADC-CoD1	(34)M=100MR-min_pilot-unC-CoD1		(35)M=100RZF-min_pilot-unC-CoD1	(36)M=100SMMSE-min_pilot-unC-CoD1	(37)M=100MR-min_pilot-ADC-CoDK		(38)M=100RZF-min_pilot-ADC-CoDK		(39)M=100SMMSE-min_pilot-ADC-CoDK	(40)M=100MR-min_pilot-unC-CoDK		(41)M=100RZF-min_pilot-unC-CoDK		(42)M=100SMMSE-min_pilot-unC-CoDK	(43)M=100MR-min_pilot-ADC-Cfree	(44)M=100RZF-min_pilot-ADC-Cfree	(45)M=100SMMSE-min_pilot-ADC-Cfree	(46)M=100MR-min_pilot-unC-Cfree		(47)M=100RZF-min_pilot-unC-Cfree	(48)M=100SMMSE-min_pilot-unC-Cfree	(49)M=100Cl_form-Eq-bit--CoI		(50)M=100Cl_form-Eq-bit--CoD1		(51)M=100Cl_form-Eq-bit--CoDK	(52)M=100Cl_form-Eq-bit--Cfree		(53)M=100Cl_form-min_pilot--CoI		(54)M=100Cl_form-min_pilot--CoD1	(55)M=100Cl_form-min_pilot--CoDK	(56)M=100Cl_form-min_pilot--Cfree	

==> Figures/CDF_minPilotQbit_RZF.tex <==
% !TeX root = ../HWI_OP_draft.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8


\begin{tikzpicture}
	%\usetikzlibrary{arrows}
	\begin{axis}[
	width=0.47\textwidth,
	height=0.32\textwidth,
	y label style = {at={(-0.03,0.5)},anchor=north},
	xlabel={SE per UE [bpcu]},
	ylabel={CDF},
%	extra y ticks={2},
%	extra y tick labels={2},% \footnotesize
%	extra x ticks={25},
%	extra x tick labels={25},		
	xmin = 0,
	xmax =6,
	ymin = 0,
	ymax = 1,
%	xtick distance = 100,
%	ytick distance = 10,
	line width = 1pt,
	grid=both,
	legend columns = 1,
%	transpose legend,
	%	 legend pos= north west,%(0.44,0.99)
%	legend style={at={(axis cs: 600,1.35)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	legend style={at={(axis cs: 2.5,0.95)},font=\footnotesize,line width=1pt,draw=black,mark size=0.1pt},
	]	

% ============== LEGEND ===================

	\addlegendentry{Co-corr-I}	
	\addlegendimage{black, mark=square, solid,mark options={solid, line width = 0.8pt},mark size=2pt}	
	\addlegendentry{Co-corr-D1}	
	\addlegendimage{red, mark=triangle,    densely dashed,mark options={solid, line width = 0.8pt},mark size=2pt}
	\addlegendentry{Co-corr-DK}
	\addlegendimage{green, mark=x,    dashdotdotted,mark options={solid, line width = 0.9pt},mark size=2.3pt}
	\addlegendentry{Cell-free}	
	\addlegendimage{blue, mark=o,    densely dotted,mark options={solid, line width = 0.8pt},mark size=2pt}
% ============== PLOTS ===================
% All results are for M = 100

% RZF  Eq - ADC - CoI 
	\addplot [black, mark=square, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={18}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% RZF  Eq - unCorr - CoI 
\addplot [black, mark=none, solid]%,xindexrange={3}{5} 		
table[x index={20}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
				
% RZF  Eq - ADC - CoD1								
	\addplot [red, mark=triangle, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
	table[x index={22}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			

% RZF  Eq - unCorr - CoD1
	\addplot [red, mark=none,    densely dashed]%,xindexrange={3}{5} 		
	table[x index={24}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};			


% RZF  Eq - ADC - CoDK								
	\addplot [green, mark=x, only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.9pt},mark size=2.5pt]%,xindexrange={3}{5} 		
	table[x index={26}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	
% RZF  Eq - unCorr - CoDK
	\addplot [green, mark=none,    dashdotdotted]%,xindexrange={3}{5} 		
	table[x index={28}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};	




% RZF  Eq - ADC - Cfree 
\addplot [blue, mark=o,only marks,mark repeat=10,mark phase=1,mark options={solid, line width = 0.8pt},mark size=2pt]%,xindexrange={3}{5} 		
table[x index={30}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		

% RZF  Eq - unCorr - Cfree 
\addplot [blue, mark=none, densely dotted]%,xindexrange={3}{5} 		
table[x index={32}, y index={0}] {Figures/Prct_SE_Eq_minPilot_Qbit.txt};		
%			green!60!black

	\end{axis}
	\end{tikzpicture}%
%   (0)Percentile				(1)MR-Hw-Eq-PwFx-ADC-CoI	(2)RZF-Hw-Eq-PwFx-ADC-CoI		(3)MR-Hw-Eq-PwFx-unC-CoI	(4)RZF-Hw-Eq-PwFx-unC-CoI		(5)MR-Hw-Eq-PwFx-ADC-CoD1	(6)RZF-Hw-Eq-PwFx-ADC-CoD1		(7)MR-Hw-Eq-PwFx-unC-CoD1	(8)RZF-Hw-Eq-PwFx-unC-CoD1		(9)MR-Hw-Eq-PwFx-ADC-CoDK	(10)RZF-Hw-Eq-PwFx-ADC-CoDK		(11)MR-Hw-Eq-PwFx-unC-CoDK	(12)RZF-Hw-Eq-PwFx-unC-CoDK		(13)MR-Hw-Eq-PwFx-ADC-Cfree	(14)RZF-Hw-Eq-PwFx-ADC-Cfree	(15)MR-Hw-Eq-PwFx-unC-Cfree	(16)RZF-Hw-Eq-PwFx-unC-Cfree	(17)MR-Hw-mPi-PwFx-ADC-CoI	(18)RZF-Hw-mPi-PwFx-ADC-CoI		(19)MR-Hw-mPi-PwFx-unC-CoI	(20)RZF-Hw-mPi-PwFx-unC-CoI		(21)MR-Hw-mPi-PwFx-ADC-CoD1	(22)RZF-Hw-mPi-PwFx-ADC-CoD1	(23)MR-Hw-mPi-PwFx-unC-CoD1	(24)RZF-Hw-mPi-PwFx-unC-CoD1	(25)MR-Hw-mPi-PwFx-ADC-CoDK	(26)RZF-Hw-mPi-PwFx-ADC-CoDK	(27)MR-Hw-mPi-PwFx-unC-CoDK	(28)RZF-Hw-mPi-PwFx-unC-CoDK	(29)MR-Hw-mPi-PwFx-ADC-Cfree	(30)RZF-Hw-mPi-PwFx-ADC-Cfree	(31)MR-Hw-mPi-PwFx-unC-Cfree	(32)RZF-Hw-mPi-PwFx-unC-Cfree	(33)Cl_form-Hw-Eq-PwFx--CoI	(34)Cl_form-Hw-Eq-PwFx--CoD1	(35)Cl_form-Hw-Eq-PwFx--CoDK	(36)Cl_form-Hw-Eq-PwFx--Cfree	(37)Cl_form-Hw-mPi-PwFx--CoI	(38)Cl_form-Hw-mPi-PwFx--CoD1	(39)Cl_form-Hw-mPi-PwFx--CoDK	(40)Cl_form-Hw-mPi-PwFx--Cfree		

%==========================================================
%   (0)Percentile					(1)M=100MR-Eq-bit-ADC-CoI			(2)M=100RZF-Eq-bit-ADC-CoI			(3)M=100SMMSE-Eq-bit-ADC-CoI	(4)M=100MR-Eq-bit-unC-CoI			(5)M=100RZF-Eq-bit-unC-CoI			(6)M=100SMMSE-Eq-bit-unC-CoI		(7)M=100MR-Eq-bit-ADC-CoD1	(8)M=100RZF-Eq-bit-ADC-CoD1			(9)M=100SMMSE-Eq-bit-ADC-CoD1		(10)M=100MR-Eq-bit-unC-CoD1			(11)M=100RZF-Eq-bit-unC-CoD1	(12)M=100SMMSE-Eq-bit-unC-CoD1		(13)M=100MR-Eq-bit-ADC-CoDK			(14)M=100RZF-Eq-bit-ADC-CoDK		(15)M=100SMMSE-Eq-bit-ADC-CoDK	(16)M=100MR-Eq-bit-unC-CoDK			(17)M=100RZF-Eq-bit-unC-CoDK		(18)M=100SMMSE-Eq-bit-unC-CoDK		(19)M=100MR-Eq-bit-ADC-Cfree	(20)M=100RZF-Eq-bit-ADC-Cfree		(21)M=100SMMSE-Eq-bit-ADC-Cfree		(22)M=100MR-Eq-bit-unC-Cfree		(23)M=100RZF-Eq-bit-unC-Cfree	(24)M=100SMMSE-Eq-bit-unC-Cfree		(25)M=100MR-min_pilot-ADC-CoI		(26)M=100RZF-min_pilot-ADC-CoI		(27)M=100SMMSE-min_pilot-ADC-CoI	(28)M=100MR-min_pilot-unC-CoI		(29)M=100RZF-min_pilot-unC-CoI		(30)M=100SMMSE-min_pilot-unC-CoI	(31)M=100MR-min_pilot-ADC-CoD1	(32)M=100RZF-min_pilot-ADC-CoD1		(33)M=100SMMSE-min_pilot-ADC-CoD1	(34)M=100MR-min_pilot-unC-CoD1		(35)M=100RZF-min_pilot-unC-CoD1	(36)M=100SMMSE-min_pilot-unC-CoD1	(37)M=100MR-min_pilot-ADC-CoDK		(38)M=100RZF-min_pilot-ADC-CoDK		(39)M=100SMMSE-min_pilot-ADC-CoDK	(40)M=100MR-min_pilot-unC-CoDK		(41)M=100RZF-min_pilot-unC-CoDK		(42)M=100SMMSE-min_pilot-unC-CoDK	(43)M=100MR-min_pilot-ADC-Cfree	(44)M=100RZF-min_pilot-ADC-Cfree	(45)M=100SMMSE-min_pilot-ADC-Cfree	(46)M=100MR-min_pilot-unC-Cfree		(47)M=100RZF-min_pilot-unC-Cfree	(48)M=100SMMSE-min_pilot-unC-Cfree	(49)M=100Cl_form-Eq-bit--CoI		(50)M=100Cl_form-Eq-bit--CoD1		(51)M=100Cl_form-Eq-bit--CoDK	(52)M=100Cl_form-Eq-bit--Cfree		(53)M=100Cl_form-min_pilot--CoI		(54)M=100Cl_form-min_pilot--CoD1	(55)M=100Cl_form-min_pilot--CoDK	(56)M=100Cl_form-min_pilot--Cfree	
